A Hamiltonian and geometric formulation of general Vlasov-Maxwell-type models

Three geometric formulations of the Hamiltonian structure of the macroscopic Maxwell equations are given: one in terms of the double de Rham complex, one in terms of L2 duality, and one utilizing an abstract notion of duality. The final of these is used to express the geometric and Hamiltonian structure of kinetic theories in general media. The Poisson bracket so stated is explicitly metric free. Finally, as a special case, the Lorentz covariance of such kinetic theories is investigated. We obtain a Lorentz covariant kinetic theory coupled to nonlinear electrodynamics such as Born-Infeld or Euler-Heisenberg electrodynamics.

==> sections/maxwell-lorentz-transformations.tex <==
%------------------------------------------------------------------------------------------------------------------------------------------------%
%-----------------Macroscopic Maxwell equations under Lorentz Transformations-------------------------------------------%
%------------------------------------------------------------------------------------------------------------------------------------------------%
\section{Macroscopic Maxwell equations under Lorentz Transformations}
We now consider the invariance of the macroscopic Maxwell equations under Lorentz transformations. One may show that position and time transform as 
\begin{equation}
	\begin{aligned}
		\bm{r}' &= \bm{r} - \gamma \bm{v} t + (\gamma - 1) \frac{(\bm{r} \cdot \bm{v})}{v^2} \bm{v}, \\
		t' &= \gamma \left( t - \frac{\bm{r} \cdot \bm{v}}{c^2} \right),
	\end{aligned}
\end{equation}
the current and charge densities transform as
\begin{equation}
	\begin{aligned}
		\bm{J}' &= \bm{J} - \gamma \bm{v} \rho + (\gamma - 1) \frac{(\bm{J} \cdot \bm{v})}{v^2} \bm{v}, \\
		\rho' &= \gamma \left( \rho - \frac{\bm{J} \cdot \bm{v}}{c^2} \right),
	\end{aligned}
\end{equation}
the $(\bm{E}, \bm{B})$ fields transform as
\begin{equation}
	\begin{aligned}
		\bm{E}' &= \gamma ( \bm{E} + \bm{v} \times \bm{B} ) + (1 - \gamma) \frac{\bm{E} \cdot \bm{v}}{v^2} \bm{v}, \\
		\bm{B}' &= \gamma \left( \bm{B} - \frac{1}{c^2} \bm{v} \times \bm{E} \right) + ( 1 - \gamma) \frac{\bm{B} \cdot \bm{v}}{v^2} \bm{v},
	\end{aligned}
\end{equation}
and the $(\bm{D}, \bm{H})$ fields transform as
\begin{equation}
	\begin{aligned}
		\bm{D}' &= \gamma \left( \bm{D} + \frac{1}{c^2} \bm{v} \times \bm{H} \right) + ( 1 - \gamma) \frac{\bm{D} \cdot \bm{v}}{v^2} \bm{v}, \\
		\bm{H}' &= \gamma ( \bm{H} - \bm{v} \times \bm{D} ) + (1 - \gamma) \frac{\bm{H} \cdot \bm{v}}{v^2} \bm{v}.
	\end{aligned}
\end{equation}
Hence, we can see that the polarization and magnetization must transform in a like manner: 
\begin{equation}
	\begin{aligned}
		\bm{P}' &= \gamma \left( \bm{P} + \frac{1}{c^2} \bm{v} \times \bm{M} \right) + ( 1 - \gamma) \frac{\bm{P} \cdot \bm{v}}{v^2} \bm{v}, \\
		\bm{M}' &= \gamma ( \bm{M} - \bm{v} \times \bm{P} ) + (1 - \gamma) \frac{\bm{M} \cdot \bm{v}}{v^2} \bm{v}.
	\end{aligned}
\end{equation}
These conditions ensure the invariance of the macroscopic Maxwell equations with respect to Lorentz transformations. In the following, we shall show that the macroscopic Maxwell equations (without free charge or current densities) possess this invariant structure when expressed as a Hamiltonian field theory. 

To begin, note that the Lorentz boost to the fields may be written
\begin{equation}
	\begin{pmatrix}
		\bm{E}' \\
		\bm{B}'
	\end{pmatrix}
		=
	\begin{pmatrix}
		\gamma \mathbb{I} + (1 - \gamma) \dfrac{\bm{v} \otimes \bm{v}}{v^2} & \gamma \hat{\bm{v}} \\
		- \dfrac{\gamma}{c^2} \hat{\bm{v}} & \gamma \mathbb{I} + (1 - \gamma) \dfrac{\bm{v} \otimes \bm{v}}{v^2} 
	\end{pmatrix}
	\begin{pmatrix}
		\bm{E} \\
		\bm{B}
	\end{pmatrix}
		=: \mathbb{B}(\bm{v})
	\begin{pmatrix}
		\bm{E} \\
		\bm{B}
	\end{pmatrix}
\end{equation}
where the hat indicates $\hat{\bm{v}} \bm{F} = \bm{v} \times \bm{F}$. Note, this reduces to just the identity for fields parallel to the boost, so we concern ourselves with the perpendicular components. In that case, the transformation is simply
\begin{equation}
	\begin{pmatrix}
		\bm{E}_\perp' \\
		\bm{B}_\perp'
	\end{pmatrix}
		=
	\gamma \begin{pmatrix}
		\mathbb{I} & \hat{\bm{v}} \\
		- \dfrac{1}{c^2} \hat{\bm{v}} &\mathbb{I} 
	\end{pmatrix}
	\begin{pmatrix}
		\bm{E}_\perp \\
		\bm{B}_\perp
	\end{pmatrix}.
\end{equation}
Clearly,
\begin{equation}
	\gamma^2 
	\begin{pmatrix}
		\mathbb{I} & \hat{\bm{v}} \\
		- \dfrac{1}{c^2} \hat{\bm{v}} &\mathbb{I} 
	\end{pmatrix}
	\begin{pmatrix}
		\mathbb{I} & -\hat{\bm{v}} \\
		\dfrac{1}{c^2} \hat{\bm{v}} &\mathbb{I} 
	\end{pmatrix}
	=
	\begin{pmatrix}
		\mathbb{I} & 0 \\
		0 & \mathbb{I}
	\end{pmatrix}.
\end{equation}
Hence, we find that $\mathbb{B}^{-1}(\bm{v}) = \mathbb{B}(- \bm{v})$. 

Now, suppose $K = K[\bm{E}, \bm{B}]$. Moreover, let
\begin{equation}
	\bm{P} = - \frac{\delta K}{\delta \bm{E}}
	\quad \text{and} \quad
	\bm{M} = \frac{\delta K}{\delta \bm{B}}.
\end{equation}
Hence, if $\overline{K}[\bm{E}', \bm{B}'] = K[\bm{E}, \bm{B}]$, we find that
\begin{equation}
	\begin{aligned}
		\frac{\delta K}{\delta ( \bm{E}, \bm{B} )} \cdot ( \delta \bm{E}, \delta \bm{B} ) 
			&= \frac{\delta \overline{K}}{\delta ( \bm{E}', \bm{B}'  )} \cdot ( \delta \bm{E}', \delta \bm{B}' ) \\
			&= \frac{\delta \overline{K}}{\delta ( \bm{E}', \bm{B}'  )} \cdot \mathbb{B}(\bm{v}) ( \delta \bm{E}, \delta \bm{B} ) \\
			&= \mathbb{B}^T(\bm{v}) \frac{\delta \overline{K}}{\delta ( \bm{E}', \bm{B}'  )} ( \delta \bm{E}, \delta \bm{B} )
	\end{aligned}
\end{equation}
which implies
\begin{equation}
	\begin{pmatrix}
		-\bm{P}' \\
		\bm{M}'
	\end{pmatrix}
		=
	\frac{\delta \overline{K}}{\delta ( \bm{E}', \bm{B}'  )} = \mathbb{B}^{-T}(\bm{v}) \frac{\delta K}{\delta ( \bm{E}, \bm{B} )}
		=
	\mathbb{B}^{-T}(\bm{v})
	\begin{pmatrix}
		-\bm{P} \\
		\bm{M}
	\end{pmatrix}.
\end{equation}
But
\begin{equation}
	\mathbb{B}^{-T}(\bm{v}) 
		=
	\mathbb{B}^{T}(-\bm{v}) 
		=
	\begin{pmatrix}
		\gamma \mathbb{I} + (1 - \gamma) \dfrac{\bm{v} \otimes \bm{v}}{v^2} & -\dfrac{\gamma}{c^2} \hat{\bm{v}} \\
		\gamma \hat{\bm{v}} & \gamma \mathbb{I} + (1 - \gamma) \dfrac{\bm{v} \otimes \bm{v}}{v^2} 
	\end{pmatrix}
\end{equation}
since $\hat{\bm{v}}^T = \hat{\bm{v}}$. Hence,
\begin{equation}
	\begin{aligned}
		\begin{pmatrix}
			-\bm{P}' \\
			\bm{M}'
		\end{pmatrix}
			&=
		\begin{pmatrix}
			\gamma \mathbb{I} + (1 - \gamma) \dfrac{\bm{v} \otimes \bm{v}}{v^2} & -\dfrac{\gamma}{c^2} \hat{\bm{v}} \\
			\gamma \hat{\bm{v}} & \gamma \mathbb{I} + (1 - \gamma) \dfrac{\bm{v} \otimes \bm{v}}{v^2} 
		\end{pmatrix}
		\begin{pmatrix}
			-\bm{P} \\
			\bm{M}
		\end{pmatrix} \\
			&=
		\begin{pmatrix}
			\gamma(-\bm{P} - \dfrac{1}{c^2} \bm{v} \times \bm{M}) - (1 - \gamma) \dfrac{\bm{v} \cdot \bm{P}}{v^2} \bm{v} \\
			\gamma(\bm{M} - \bm{v} \times \bm{P}) + (1 - \gamma) \dfrac{\bm{v} \cdot \bm{M}}{v^2} \bm{v}
		\end{pmatrix}.
	\end{aligned}
\end{equation}
Simplifying this, we obtain the desired result:
\begin{equation}
	\begin{aligned}
		\bm{P}' &= \gamma(\bm{P} + \dfrac{1}{c^2} \bm{v} \times \bm{M}) + (1 - \gamma) \dfrac{\bm{v} \cdot \bm{P}}{v^2} \bm{v} \\
		\bm{M}' &= \gamma(\bm{M} - \bm{v} \times \bm{P}) + (1 - \gamma) \dfrac{\bm{v} \cdot \bm{M}}{v^2} \bm{v}.
	\end{aligned}
\end{equation}
Therefore, the polarization and magnetization fields defined as the gradients of a general energy functional transform as needed for the macroscopic Maxwell equations to be invariant under Lorentz transformations. 

Hence, if 
\begin{equation}
	\begin{pmatrix}
		\bm{D} \\
		\bm{H}
	\end{pmatrix}
		= 
		\mathcal{R}
	\begin{pmatrix}
		\bm{E} \\
		\bm{B} 
	\end{pmatrix}
		+ 4 \pi
	\begin{pmatrix}
		 - \delta K / \delta \bm{E}, \\
		 \delta K / \delta \bm{B}
	\end{pmatrix}
\end{equation}
where $\mathcal{R}$ indicates the Riesz map which maps the vector fields $(\bm{E}, \bm{B})$ to their dual representation. To find out how how these transform, we write the following:
\begin{equation}
	\left(
	\begin{pmatrix}
		\bm{E} \\
		\bm{B}
	\end{pmatrix}
	,
	\begin{pmatrix}
		\delta \bm{E} \\
		\delta \bm{B}
	\end{pmatrix}
	\right)
	= 
	\left(
	\begin{pmatrix}
		\bm{E}' \\
		\bm{B}'
	\end{pmatrix}
	,
	\begin{pmatrix}
		\delta \bm{E}' \\
		\delta \bm{B}'
	\end{pmatrix}
	\right)
	=
	\left(
	\begin{pmatrix}
		\bm{E}' \\
		\bm{B}'
	\end{pmatrix}
	,
	\mathbb{B}(\bm{v})
	\begin{pmatrix}
		\delta \bm{E} \\
		\delta \bm{B}
	\end{pmatrix}
	\right).
\end{equation}
Hence, we see that $\mathcal{R} (\bm{E}', \bm{B}') = \mathbb{B}^{-T}(\bm{v}) \mathcal{R} (\bm{E}, \bm{B})$ just as $(\bm{P}, \bm{M})$ transform. Hence, we find that
\begin{equation}
	\begin{aligned}
		\bm{D}' &= \gamma(\bm{D} + \dfrac{1}{c^2} \bm{v} \times \bm{H}) + (1 - \gamma) \dfrac{\bm{v} \cdot \bm{D}}{v^2} \bm{v} \\
		\bm{H}' &= \gamma(\bm{H} - \bm{v} \times \bm{D}) + (1 - \gamma) \dfrac{\bm{v} \cdot \bm{H}}{v^2} \bm{v}
	\end{aligned}
\end{equation}
as desired. 

